Beyond Token-Local Imitation: Reward-Compatible Temporal Credit Assignment for On-Policy Distillation

On-policy distillation (OPD) has emerged as an effective approach for large language model post-training, yet existing objectives face a trade-off between objective fidelity and optimization stability. Token-level OPD provides stable but local supervision, whereas sequence-level OPD captures future credit at the cost of horizon-dependent variance. We establish a unified temporal-credit view of these formulations, showing that practical token-level OPD can be interpreted as a temporal approximation to the sequence-level reverse-KL gradient. Building on this connection, we propose $\gamma$OPD (GammaOPD), which uses discounted temporal credit assignment to balance long-horizon supervision and optimization stability, while admitting a horizon-independent variance bound. We further develop a reward-compatible bounded mixing (RBM) mechanism for $\gamma$OPD that balances verifiable outcome feedback with the discounted OPD advantage to move beyond purely teacher-dependent optimization. Experiments on mathematical and code reasoning demonstrate consistent improvements over existing OPD methods across vanilla, size-mismatched, and multi-teacher distillation settings.

==> author_commands.tex <==
% Author and affiliation formatting for the ICLR manuscript.
\makeatletter
\let\iclrstandardauthor\author
\newcommand{\iclrmaybeauthorsup}[1]{%
  \if\relax\detokenize{#1}\relax
  \else
    \textsuperscript{#1}%
  \fi
}
\newcommand{\iclr@authorlist}{}
\newcommand{\iclr@affiliationlist}{}
\newcommand{\iclr@contributionlist}{}
\newcommand{\iclrAuthorBlockWidth}{0.96\textwidth}
\newcommand{\iclrTitleAuthorGap}{1.2ex}
\newcommand{\iclrAuthorAffiliationGap}{0.9ex}
\newcommand{\iclrAffiliationContributionGap}{0.7ex}
\newcommand{\iclrAuthorLineSpread}{1.12}
\newif\ificlr@firstauthor
\newif\ificlr@firstaffiliation
\newif\ificlr@firstcontribution
\iclr@firstauthortrue
\iclr@firstaffiliationtrue
\iclr@firstcontributiontrue
\renewcommand{\author}[2][]{%
  \ificlr@firstauthor
    \global\iclr@firstauthorfalse
  \else
    \g@addto@macro\iclr@authorlist{, }%
  \fi
  \g@addto@macro\iclr@authorlist{#2\iclrmaybeauthorsup{#1}}%
}
\newcommand{\affiliation}[2][]{%
  \ificlr@firstaffiliation
    \global\iclr@firstaffiliationfalse
  \else
    \g@addto@macro\iclr@affiliationlist{\\}%
  \fi
  \g@addto@macro\iclr@affiliationlist{\iclrmaybeauthorsup{#1}#2}%
}
\newcommand{\contribution}[2][]{%
  \ificlr@firstcontribution
    \global\iclr@firstcontributionfalse
  \else
    \g@addto@macro\iclr@contributionlist{\qquad}%
  \fi
  \g@addto@macro\iclr@contributionlist{\iclrmaybeauthorsup{#1}#2}%
}
\AtBeginDocument{%
  \iclrstandardauthor{%
    \parbox{\iclrAuthorBlockWidth}{\centering
      \mbox{}\\[\iclrTitleAuthorGap]
      {\linespread{\iclrAuthorLineSpread}\selectfont\normalsize \iclr@authorlist}%
      \\[\iclrAuthorAffiliationGap]
      {\normalfont\small \iclr@affiliationlist}%
      \ificlr@firstcontribution
      \else
        \\[\iclrAffiliationContributionGap]
        {\normalfont\small \iclr@contributionlist}%
      \fi
    }%
  }%
}
\makeatother


==> iclr2027_mode_commands.tex <==
% Optional author-visible preprint mode for the official ICLR 2027 style.
%
% The submission path remains untouched: with no mode command enabled,
% iclr2027_conference.sty provides the official anonymous format and line
% numbers.  This file only supplies a backwards-compatible, opt-in command
% for producing an arXiv/preprint PDF from the same source.
\RequirePackage{etoolbox}
\makeatletter
\newif\ificlrpreprint
\iclrpreprintfalse
\newcommand{\iclrpreprintcopy}{%
  \iclrfinalcopy
  \iclrpreprinttrue
  \patchcmd{\@maketitle}%
    {\lhead{Published as a conference paper at ICLR 2027}}%
    {\lhead{Preprint}}{}{}%
}
\makeatother

